Interpretable bias mitigation for textual data: Reducing gender bias in patient notes while maintaining classification performance

Medical systems in general, and patient treatment decisions and outcomes in particular, are affected by bias based on gender and other demographic elements. As language models are increasingly applied to medicine, there is a growing interest in building algorithmic fairness into processes impacting patient care. Much of the work addressing this question has focused on biases encoded in language models -- statistical estimates of the relationships between concepts derived from distant reading of corpora. Building on this work, we investigate how word choices made by healthcare practitioners and language models interact with regards to bias. We identify and remove gendered language from two clinical-note datasets and describe a new debiasing procedure using BERT-based gender classifiers. We show minimal degradation in health condition classification tasks for low- to medium-levels of bias removal via data augmentation. Finally, we compare the bias semantically encoded in the language models with the bias empirically observed in health records. This work outlines an interpretable approach for using data augmentation to identify and reduce the potential for bias in natural language processing pipelines.

==> tables/i2b2_rtd_rtd.tex <==
\begin{table}[ht!]
\centering
\rowcolors{2}{lightgray}{white}
\begin{tabular}{|l|l|r|r|r|}
\toprule
\hline
{} & 1gram & 
\begin{tabular}{@{}c@{}}BERT \\ RTD rank\end{tabular}   & 
\begin{tabular}{@{}c@{}}\iibb  \\ RTD rank\end{tabular} &  
\begin{tabular}{@{}c@{}}BERT-\iibb \\ RTD rank\end{tabular}
 \\
\hline
\midrule
1  &        mrs &       1.0 &    1172.5 &      1.0 \\
2  &         ms &       4.0 &    6560.5 &      2.0 \\
3  &        her &     279.0 &       3.0 &      3.0 \\
4  &        mr. &   15307.0 &       6.0 &      4.0 \\
5  &       male &   21798.0 &       8.0 &      5.0 \\
6  &         mr &       5.0 &     437.0 &      6.0 \\
7  &     female &    5150.0 &       9.0 &      7.0 \\
8  &      linda &      10.0 &    3681.5 &      8.0 \\
9  &        ms. &    2208.0 &      11.0 &      9.0 \\
10 &  gentleman &    3054.0 &      13.0 &     10.0 \\
11 &        pap &   25105.0 &      17.0 &     11.0 \\
12 &     breast &    4314.0 &      14.0 &     12.0 \\
13 &   cervical &      14.0 &    2483.0 &     13.0 \\
14 &    biggest &      16.0 &    5301.5 &     14.0 \\
15 &  mammogram &   25054.0 &      21.0 &     15.0 \\
16 &       mrs. &    2860.0 &      16.0 &     16.0 \\
17 &          f &   10458.0 &      20.0 &     17.0 \\
18 &      woman &     120.0 &       7.0 &     18.0 \\
19 &        psa &    6082.0 &      19.0 &     19.0 \\
20 &      kathy &      19.0 &    5301.5 &     20.0 \\
21 &         he &       3.0 &       1.0 &     21.0 \\
22 &       them &      20.0 &    4146.0 &     22.0 \\
23 &   prostate &    2223.0 &      18.0 &     23.0 \\
24 &        bph &    8601.0 &      23.0 &     24.0 \\
25 &    husband &     920.0 &      15.0 &     25.0 \\
26 &        guy &      22.0 &    5301.5 &     26.0 \\
27 &       take &    4278.0 &      22.0 &     27.0 \\
28 &   infected &      18.0 &    1455.0 &     28.0 \\
29 &   patricia &      21.0 &    2701.5 &     29.0 \\
30 &      smear &   21455.0 &      29.0 &     30.0 \\
31 &      ellen &      24.0 &    3681.5 &     31.0 \\
32 &       cabg &   19064.0 &      33.0 &     32.0 \\
33 &     distal &    7754.0 &      30.0 &     33.0 \\
34 &       pend &   22515.0 &      36.0 &     34.0 \\
35 &     tablet &    2322.0 &      25.0 &     35.0 \\
36 &       cath &    7111.0 &      31.0 &     36.0 \\
37 &       qday &   12829.0 &      34.0 &     37.0 \\
38 &      peggy &      17.0 &     485.0 &     38.0 \\
39 &     flomax &   17413.0 &      37.5 &     39.0 \\
40 &        lad &    2383.0 &      27.0 &     40.0 \\
41 &  prostatic &   23978.0 &      43.0 &     41.0 \\
42 &       gout &   11948.0 &      40.0 &     42.0 \\
43 &     taking &    9534.0 &      39.0 &     43.0 \\
44 &    trouble &      34.0 &    4183.5 &     44.0 \\
45 &      harry &      33.0 &    3372.0 &     45.0 \\
46 &    vaginal &   10418.0 &      41.0 &     46.0 \\
47 &        qty &   18645.0 &      45.0 &     47.0 \\
48 &        she &       6.0 &       2.0 &     48.0 \\
49 &        p.o &    9293.0 &      42.0 &     49.0 \\
50 &        xie &   20584.0 &      47.5 &     50.0 \\
\hline
\bottomrule
\end{tabular}
\caption{\textbf{Rank-turbulence divergence of the rank-turbulence divergence between male and female Zipf distributions according to i2b2 rank-turbulence divergence and BERT cosine similarity ranking. }}
\label{tab:i2b2_rtd_rtd}
\end{table}

==> tables/rtd2_BERT.tex <==
\begin{table*}[ht!]

\centering
\rowcolors{2}{lightgray}{white}
\begin{tabular}{|l|r|r|r|r|r|}

\toprule
\hline
1gram &  
\begin{tabular}{@{}c@{}}BERT \\ RTD rank\end{tabular} &  
\begin{tabular}{@{}c@{}}MIMIC \\ RTD rank\end{tabular} &  \begin{tabular}{@{}c@{}}BERT-MIMC \\ RTD rank\end{tabular} &  \begin{tabular}{@{}c@{}}MIMIC \\ F rank\end{tabular} &
\begin{tabular}{@{}c@{}}MIMIC \\ M rank\end{tabular} \\
\midrule
\hline
sexually       &            2.0 &         16755.5 &           1.0 &      10607.0 &    10373.5 \\
biggest        &            3.0 &          7594.5 &           2.0 &      17520.5 &    21172.5 \\
f              &         6288.0 &             3.0 &           3.0 &        251.0 &     1719.0 \\
infected       &            5.0 &         16076.0 &           4.0 &       3475.0 &     3402.5 \\
grandmother    &            4.0 &          3517.0 &           5.0 &       6090.0 &     7643.0 \\
cervical       &            7.0 &         18374.0 &           6.0 &       1554.0 &     1551.5 \\
m              &          244.0 &             2.0 &           7.0 &       2103.0 &      249.0 \\
sister         &            6.0 &          4153.0 &           8.0 &       1213.5 &     1365.0 \\
husband        &          860.0 &             4.0 &           9.0 &        495.0 &     5114.0 \\
teenage        &            9.0 &          5513.0 &          10.0 &      15449.0 &    19594.0 \\
trouble        &           12.0 &         10119.0 &          11.0 &       3778.5 &     4095.5 \\
brother        &           10.0 &          1921.0 &          12.0 &       1925.0 &     1598.0 \\
teenager       &            8.0 &           936.5 &          13.0 &      12928.5 &    21172.5 \\
connected      &           16.0 &         16682.0 &          14.0 &       5184.5 &     5089.5 \\
shaky          &           11.0 &          2341.0 &          15.0 &      10607.0 &     7872.0 \\
my             &           15.0 &          8198.0 &          16.0 &       2395.0 &     2624.5 \\
breast         &         3397.0 &             6.0 &          17.0 &       1075.0 &     4673.5 \\
expelled       &           19.0 &         14652.5 &          18.0 &      20814.0 &    19594.0 \\
them           &           18.0 &         11337.0 &          19.0 &       1738.5 &     1832.0 \\
prostate       &         2196.0 &             5.0 &          20.0 &       9436.0 &     1576.5 \\
immune         &           20.0 &         15043.5 &          21.0 &       9119.0 &     8753.0 \\
daughter       &            1.0 &            16.0 &          22.0 &        463.0 &      801.5 \\
initial        &           23.0 &         11433.0 &          23.0 &        632.5 &      610.0 \\
ovarian        &        16374.0 &             8.0 &          24.0 &       3137.0 &    14082.0 \\
recovering     &           24.0 &         11867.0 &          25.0 &       5351.5 &     5749.5 \\
abnormal       &           25.0 &          9010.0 &          26.0 &       1849.5 &     1994.0 \\
alcoholic      &           17.0 &          1136.0 &          27.0 &       3885.5 &     2952.0 \\
obvious        &           26.0 &         10154.0 &          28.0 &       2725.5 &     2540.5 \\
huge           &           28.0 &         13683.5 &          29.0 &       8069.0 &     7643.0 \\
dirty          &           29.0 &         13264.5 &          30.0 &       8613.5 &     9179.5 \\
suv            &           27.0 &          5911.0 &          31.0 &      14704.0 &    18377.5 \\
container      &           31.0 &         17776.0 &          32.0 &      12090.5 &    12214.5 \\
flomax         &        10891.0 &            11.0 &          33.0 &      17520.5 &     4095.5 \\
sisters        &           32.0 &         17680.5 &          34.0 &       4727.0 &     4687.5 \\
uterine        &         7260.0 &            10.0 &          35.0 &       4263.0 &    19594.0 \\
hypothyroidism &        17831.0 &            12.0 &          36.0 &       1239.5 &     2920.0 \\
dried          &     sexually       &            2.0 &         16755.5 &           1.0 &      10607.0 &    10373.5 \\
biggest        &            3.0 &          7594.5 &           2.0 &      17520.5 &    21172.5 \\
f              &         6288.0 &             3.0 &           3.0 &        251.0 &     1719.0 \\
infected       &            5.0 &         16076.0 &           4.0 &       3475.0 &     3402.5 \\
grandmother    &            4.0 &          3517.0 &           5.0 &       6090.0 &     7643.0 \\
cervical       &            7.0 &         18374.0 &           6.0 &       1554.0 &     1551.5 \\
m              &          244.0 &             2.0 &           7.0 &       2103.0 &      249.0 \\
sister         &            6.0 &          4153.0 &           8.0 &       1213.5 &     1365.0 \\
husband        &          860.0 &             4.0 &           9.0 &        495.0 &     5114.0 \\
teenage        &            9.0 &          5513.0 &          10.0 &      15449.0 &    19594.0 \\
trouble        &           12.0 &         10119.0 &          11.0 &       3778.5 &     4095.5 \\
brother        &           10.0 &          1921.0 &          12.0 &       1925.0 &     1598.0 \\
teenager       &            8.0 &           936.5 &          13.0 &      12928.5 &    21172.5 \\
connected      &           16.0 &         16682.0 &          14.0 &       5184.5 &     5089.5 \\
shaky          &           11.0 &          2341.0 &          15.0 &      10607.0 &     7872.0 \\
my             &           15.0 &          8198.0 &          16.0 &       2395.0 &     2624.5 \\
breast         &         3397.0 &             6.0 &          17.0 &       1075.0 &     4673.5 \\
expelled       &           19.0 &         14652.5 &          18.0 &      20814.0 &    19594.0 \\
them           &           18.0 &         11337.0 &          19.0 &       1738.5 &     1832.0 \\
prostate       &         2196.0 &             5.0 &          20.0 &       9436.0 &     1576.5 \\
immune         &           20.0 &         15043.5 &          21.0 &       9119.0 &     8753.0 \\
daughter       &            1.0 &            16.0 &          22.0 &        463.0 &      801.5 \\
initial        &           23.0 &         11433.0 &          23.0 &        632.5 &      610.0 \\
ovarian        &        16374.0 &             8.0 &          24.0 &       3137.0 &    14082.0 \\
recovering     &           24.0 &         11867.0 &          25.0 &       5351.5 &     5749.5 \\
abnormal       &           25.0 &          9010.0 &          26.0 &       1849.5 &     1994.0 \\
alcoholic      &           17.0 &          1136.0 &          27.0 &       3885.5 &     2952.0 \\
obvious        &           26.0 &         10154.0 &          28.0 &       2725.5 &     2540.5 \\
huge           &           28.0 &         13683.5 &          29.0 &       8069.0 &     7643.0 \\
dirty          &           29.0 &         13264.5 &          30.0 &       8613.5 &     9179.5 \\
suv            &           27.0 &          5911.0 &          31.0 &      14704.0 &    18377.5 \\
container      &           31.0 &         17776.0 &          32.0 &      12090.5 &    12214.5 \\
flomax         &        10891.0 &            11.0 &          33.0 &      17520.5 &     4095.5 \\
sisters        &           32.0 &         17680.5 &          34.0 &       4727.0 &     4687.5 \\
uterine        &         7260.0 &            10.0 &          35.0 &       4263.0 &    19594.0 \\
hypothyroidism &        17831.0 &            12.0 &          36.0 &       1239.5 &     2920.0 \\
dried          &           34.0 &         15661.0 &          37.0 &       5124.5 &     4982.0 \\
osteoporosis   &        18010.0 &            13.0 &          38.0 &       2354.0 &     7003.0 \\
breasts        &         4727.0 &             9.0 &          39.0 &       4394.5 &    21172.5 \\
certain        &           37.0 &         18020.5 &          40.0 &       7973.0 &     8023.0 \\
i              &           30.0 &          4601.0 &          41.0 &        403.0 &      435.5 \\
restless       &           21.0 &          1144.0 &          42.0 &       1366.0 &     1123.0 \\
wife           &           13.0 &             1.0 &          43.0 &       5545.0 &      245.5 \\
sle            &         8083.0 &            14.0 &          44.0 &       3511.0 &    12504.5 \\
granddaughter  &           14.0 &           210.0 &          45.0 &       4656.5 &     7872.0 \\
localized      &           47.0 &         14357.5 &          46.0 &       6136.0 &     6405.0 \\
ciwa           &         7921.0 &            15.0 &          47.0 &       3106.5 &     1341.0 \\
honey          &           44.0 &         11076.0 &          48.0 &      10868.5 &     9861.0 \\
coronary       &        11570.0 &            18.0 &          49.0 &        560.0 &      349.0 \\
systemic       &           41.0 &          6361.0 &          50.0 &       3696.0 &     4214.0 \\
      34.0 &         15661.0 &          37.0 &       5124.5 &     4982.0 \\
osteoporosis   &        18010.0 &            13.0 &          38.0 &       2354.0 &     7003.0 \\
breasts        &         4727.0 &             9.0 &          39.0 &       4394.5 &    21172.5 \\
certain        &           37.0 &         18020.5 &          40.0 &       7973.0 &     8023.0 \\
i              &           30.0 &          4601.0 &          41.0 &        403.0 &      435.5 \\
restless       &           21.0 &          1144.0 &          42.0 &       1366.0 &     1123.0 \\
wife           &           13.0 &             1.0 &          43.0 &       5545.0 &      245.5 \\
sle            &         8083.0 &            14.0 &          44.0 &       3511.0 &    12504.5 \\
granddaughter  &           14.0 &           210.0 &          45.0 &       4656.5 &     7872.0 \\
localized      &           47.0 &         14357.5 &          46.0 &       6136.0 &     6405.0 \\
ciwa           &         7921.0 &            15.0 &          47.0 &       3106.5 &     1341.0 \\
honey          &           44.0 &         11076.0 &          48.0 &      10868.5 &     9861.0 \\
coronary       &        11570.0 &            18.0 &          49.0 &        560.0 &      349.0 \\
systemic       &           41.0 &          6361.0 &          50.0 &       3696.0 &     4214.0 \\

\bottomrule
\hline
\end{tabular}
\caption{\textbf{Comparison of rank-turbulence divergences for gendered clusters in BERT embeddings and the MIMIC patient health records text.} 
BERT RTD ranks are calculated based on cosine similarity scores for word embedding and gendered clusters (i.e., the RTD of cosine similarity score ranks relative to male and female clusters). 
MIMIC RTD ranks are for $1$-grams from male and female clinical notes. 
``BERT-MIMIC RTD rank'' is the rankings for $1$-grams based on RTD between the first two columns---we also refer to this as RTD$^2$ (ranking divergence-of-divergence).  }
\label{tab:MIMIC_rtd_rtd}
\end{table*}


==> tables/rtd2table_deprecated.tex <==
\begin{table*}[ht!]

\centering
\rowcolors{2}{lightgray}{white}
\begin{tabular}{|l|l|r|r|r|r|r|}

\toprule
\hline
{} & 1gram &  
\begin{tabular}{@{}c@{}}BERT \\ RTD rank\end{tabular} &  
\begin{tabular}{@{}c@{}}MIMIC \\ RTD rank\end{tabular} &  \begin{tabular}{@{}c@{}}BERT-MIMC \\ RTD rank\end{tabular} &  \begin{tabular}{@{}c@{}}MIMIC \\ F rank\end{tabular} &
\begin{tabular}{@{}c@{}}MIMIC \\ M rank\end{tabular} \\
\midrule
\hline
1  &               f &    2615.0 &        4.0 &      1.0 &     4816.0 &       6356.0 \\
2  &         husband &     395.0 &        3.0 &      2.0 &     1190.0 &       6175.0 \\
3  &               m &     110.0 &        2.0 &      3.0 &     6385.0 &       4255.0 \\
4  &        cervical &       2.0 &     1167.0 &      4.0 &     5267.0 &       4908.5 \\
5  &          sister &       3.0 &     1623.0 &      5.0 &     5102.0 &       5360.5 \\
6  &        infected &       4.0 &     2644.0 &      6.0 &     3447.0 &       2824.5 \\
7  &            ciwa &    3371.0 &        5.0 &      7.0 &     5551.0 &       3143.5 \\
8  &         trouble &       5.0 &     6263.5 &      8.0 &     2890.0 &       2824.5 \\
9  &          breast &    1643.0 &        6.0 &      9.0 &     2511.0 &       5360.5 \\
10 &             icd &    2291.0 &        8.0 &     10.0 &     5127.0 &       2434.5 \\
11 &         brother &       7.0 &     2883.5 &     11.0 &     4748.0 &       4979.0 \\
12 &              my &       8.0 &     3260.5 &     12.0 &     4078.0 &       4385.0 \\
13 &  hypothyroidism &    6352.0 &       11.0 &     13.0 &     3895.0 &       5347.0 \\
14 &            them &      11.0 &     6136.0 &     14.0 &     4913.0 &       4938.0 \\
15 &            etoh &    5991.0 &       12.0 &     15.0 &     6036.0 &       5590.5 \\
16 &            disp &    4051.0 &       10.0 &     16.0 &     6316.0 &       6139.0 \\
17 &         refills &    2905.0 &        9.0 &     17.0 &     6328.5 &       6156.0 \\
18 &            aicd &    6409.0 &       15.0 &     18.0 &     4143.5 &        538.0 \\
19 &       connected &      10.0 &     1861.0 &     19.0 &     2799.0 &       1713.0 \\
20 &             hiv &    3319.0 &       13.0 &     20.0 &     4871.5 &       2575.0 \\
21 &             hip &    5332.0 &       20.0 &     21.0 &     5505.5 &       5976.0 \\
22 &       alcoholic &      12.0 &     1693.0 &     22.0 &     3262.5 &       2283.5 \\
23 &             uti &    2200.0 &       16.0 &     23.0 &     4902.0 &       5721.5 \\
24 &      withdrawal &    3255.0 &       19.0 &     24.0 &     5418.5 &       4213.5 \\
25 &   levothyroxine &    6331.0 &       23.0 &     25.0 &     3928.5 &       5249.0 \\
26 &   postoperative &    4879.0 &       22.0 &     26.0 &     5820.0 &       5221.5 \\
27 &      collection &    3594.0 &       21.0 &     27.0 &     5257.5 &       3902.5 \\
28 &        restless &      13.0 &     1638.0 &     28.0 &     5538.5 &       5327.0 \\
29 &            cabg &    6539.0 &       26.0 &     29.0 &     6096.0 &       5783.0 \\
30 &   granddaughter &       9.0 &      558.5 &     30.0 &      106.5 &       1713.0 \\
31 &            wife &       6.0 &        1.0 &     31.0 &     6380.0 &       1937.5 \\
32 &         obvious &      16.0 &     4836.0 &     32.0 &     4322.5 &       4172.5 \\
33 &         initial &      15.0 &     3789.0 &     33.0 &     5986.5 &       6026.5 \\
34 &        abnormal &      17.0 &     5278.5 &     34.0 &     4489.5 &       4385.0 \\
35 &       lopressor &    3938.0 &       27.0 &     35.0 &     6385.0 &       6288.0 \\
36 &             the &     916.0 &       17.0 &     36.0 &     6610.0 &       6608.0 \\
37 &        cerebral &    1066.0 &       18.0 &     37.0 &     3509.0 &       5149.0 \\
38 &          crying &    4757.0 &       32.0 &     38.0 &      329.0 &       3492.5 \\
39 &             p.o &    2718.0 &       25.0 &     39.0 &     6148.0 &       5878.5 \\
40 &           dried &      21.0 &     6291.5 &     40.0 &     1696.5 &       1713.0 \\
41 &            q.d. &    3077.0 &       29.0 &     41.0 &     4416.0 &       1937.5 \\
42 &           final &    4500.0 &       39.0 &     42.0 &     5791.5 &       6080.0 \\
43 &      ophthalmic &    6179.0 &       44.0 &     43.0 &     2399.5 &       4454.5 \\
44 &            pmns &    5765.0 &       43.0 &     44.0 &      560.5 &       3492.5 \\
45 &        paranoid &      24.0 &     5512.5 &     45.0 &      560.5 &        538.0 \\
46 &             q.d &    2531.0 &       30.0 &     46.0 &     5538.5 &       4680.0 \\
47 &         thyroid &     381.0 &       14.0 &     47.0 &     2799.0 &       4938.0 \\
48 &         abscess &    6523.0 &       47.0 &     48.0 &     5478.5 &       4680.0 \\
49 &            diag &    5661.0 &       46.0 &     49.0 &     3386.5 &        185.0 \\
50 &           mouth &    4068.0 &       42.0 &     50.0 &     5922.5 &       6149.5 \\
\bottomrule
\hline
\end{tabular}
\caption{\textbf{Comparison of rank-turbulence divergences for gendered clusters in BERT embeddings and the MIMIC patient health records text.} 
BERT RTD ranks are calculated based on cosine similarity scores for word embedding and gendered clusters (i.e., the RTD of cosine similarity score ranks relative to male and female clusters). 
MIMIC RTD ranks are for $1$-grams from male and female clinical notes. 
``BERT-MIMIC RTD rank'' is the rankings for $1$-grams based on RTD between the first two columns---we also refer to this as RTD$^2$ (ranking divergence-of-divergence).  }
\label{tab:MIMIC_rtd_rtd}
\end{table*}

==> tables/topconds_deprecated.tex <==
\begin{table}
\rowcolors{2}{lightgray}{white}
\begin{tabular}{l|r|r|r}
\toprule
{} & \multicolumn{2}{l}{\textbf{Sex Count}} & {} \\
 \textbf{ICD Description.}  &     \textbf{ $N_\textnormal{f}$} & \textbf{$N_\textnormal{m}$} & \textbf{ $N_\textnormal{f}$/$N_\textnormal{total}$} \\ %%\multicolumn{2}{l}{\textbf{M}} \\
 \hline
     %%                                     &        &        &       \\
\midrule
 Diabetes mellitus &   3902 &   5156 &  0.43 \\
Acute kidney failure                 &   3941 &   5178 &  0.43 \\
Acute respiratory failure           &   3473 &   4024 &  0.46 \\
Atrial fibrillation                                &   5512 &   7379 &  0.43 \\
Congestive heart failure             &   6106 &   7005 &  0.47 \\
Coronary atherosclerosis &   4322 &   8107 &  0.35 \\
Esophageal reflux                                  &   2990 &   3336 &  0.47 \\
Hyperlipidemia               &   3537 &   5153 &  0.41 \\
Essential hypertension                 &   9370 &  11333 &  0.45 \\
Urinary tract infection        &   4027 &   2528 &  0.61 \\
\bottomrule
\end{tabular}
\caption{\textbf{Patient sex ratios for the top 10 conditions in \MIMIC.}
For most health conditions there is an a imbalance in the gender ratio between male and female patients.
This reflects an overall bias in the \MIMIC dataset with has more male patients.}
\label{tab:mimic_sex}
\end{table}

==> tables/topicds.tex <==
%%\begin{table*}
\rowcolors{2}{lightgray}{white}
\begin{longtable*}{|l|r|r|r|}


%%\begin{tabular}
\toprule
{} & \multicolumn{2}{l}{\textbf{Sex Count}} & \textbf{Pct. Female} \\
 \textbf{ICD Description.}  &     \textbf{ F} & \multicolumn{2}{l}{\textbf{M}} \\
 \hline
     %%                                            &         &          &          \\
\midrule
\endhead
Routine or ritual circumcision                     &     0 &   2016 &  0.00 \\
Personal history of malignant neoplasm of prostate &     0 &   1207 &  0.00 \\
Hypertrophy (benign) of prostate without urinar... &     0 &   1490 &  0.00 \\
Gout, unspecified                                  &   552 &   1530 &  0.27 \\
Alcoholic cirrhosis of liver                       &   323 &    879 &  0.27 \\
Retention of urine, unspecified                    &   283 &    737 &  0.28 \\
Intermediate coronary syndrome                     &   466 &   1197 &  0.28 \\
Chronic systolic heart failure                     &   321 &    776 &  0.29 \\
Aortocoronary bypass status                        &   896 &   2160 &  0.29 \\
Other and unspecified angina pectoris              &   330 &    770 &  0.30 \\
Paroxysmal ventricular tachycardia                 &   548 &   1263 &  0.30 \\
Chronic hepatitis C without mention of hepatic ... &   380 &    838 &  0.31 \\
Coronary atherosclerosis of unspecified type of... &   479 &   1015 &  0.32 \\
Percutaneous transluminal coronary angioplasty ... &   889 &   1836 &  0.33 \\
Portal hypertension                                &   332 &    675 &  0.33 \\
Surgical operation with anastomosis, bypass, or... &   406 &    805 &  0.34 \\
Old myocardial infarction                          &  1156 &   2122 &  0.35 \\
Coronary atherosclerosis of native coronary artery &  4322 &   8107 &  0.35 \\
Acute on chronic systolic heart failure            &   406 &    737 &  0.36 \\
Cardiac complications, not elsewhere classified    &   847 &   1496 &  0.36 \\
Atrial flutter                                     &   444 &    773 &  0.36 \\
Personal history of tobacco use                    &  1042 &   1769 &  0.37 \\
Chronic kidney disease, unspecified                &  1265 &   2170 &  0.37 \\
Pneumonitis due to inhalation of food or vomitus   &  1369 &   2311 &  0.37 \\
Obstructive sleep apnea (adult)(pediatric)         &   891 &   1489 &  0.37 \\
Tobacco use disorder                               &  1251 &   2107 &  0.37 \\
Paralytic ileus                                    &   394 &    678 &  0.37 \\
Hypertensive chronic kidney disease, unspecifie... &  1300 &   2121 &  0.38 \\
Cirrhosis of liver without mention of alcohol      &   486 &    801 &  0.38 \\
Diabetes with neurological manifestations, type... &   438 &    700 &  0.38 \\
Other primary cardiomyopathies                     &   664 &   1045 &  0.39 \\
Hyperpotassemia                                    &   874 &   1295 &  0.40 \\
Peripheral vascular disease, unspecified           &   564 &    837 &  0.40 \\
Cardiac arrest                                     &   542 &    819 &  0.40 \\
Hemorrhage complicating a procedure                &   637 &    898 &  0.41 \\
Pressure ulcer, lower back                         &   530 &    759 &  0.41 \\
Hypertensive chronic kidney disease, unspecifie... &  1091 &   1539 &  0.41 \\
Other and unspecified hyperlipidemia               &  3537 &   5153 &  0.41 \\
Pure hypercholesterolemia                          &  2436 &   3494 &  0.41 \\
Thrombocytopenia, unspecified                      &  1255 &   1810 &  0.41 \\
Subendocardial infarction, initial episode of care &  1262 &   1793 &  0.41 \\
Bacteremia                                         &   599 &    879 &  0.41 \\
Acute kidney failure with lesion of tubular nec... &   945 &   1342 &  0.41 \\
Acute and subacute necrosis of liver               &   441 &    626 &  0.41 \\
Polyneuropathy in diabetes                         &   667 &    917 &  0.42 \\
Other postoperative infection                      &   503 &    683 &  0.42 \\
Cardiogenic shock                                  &   480 &    674 &  0.42 \\
Aortic valve disorders                             &  1069 &   1481 &  0.42 \\
Pulmonary collapse                                 &   931 &   1234 &  0.43 \\
Diabetes mellitus without mention of complicati... &  3902 &   5156 &  0.43 \\
Other and unspecified coagulation defects          &   438 &    578 &  0.43 \\
Hemorrhage of gastrointestinal tract, unspecified  &   602 &    795 &  0.43 \\
Cardiac pacemaker in situ                          &   592 &    798 &  0.43 \\
Respiratory distress syndrome in newborn           &   559 &    755 &  0.43 \\
End stage renal disease                            &   836 &   1090 &  0.43 \\
Delirium due to conditions classified elsewhere    &   622 &    823 &  0.43 \\
Atrial fibrillation                                &  5512 &   7379 &  0.43 \\
Acute kidney failure, unspecified                  &  3941 &   5178 &  0.43 \\
Accidents occurring in residential institution     &   456 &    583 &  0.44 \\
Single liveborn, born in hospital, delivered by... &  1220 &   1538 &  0.44 \\
Sepsis                                             &   563 &    709 &  0.44 \\
Hyperosmolality and/or hypernatremia               &  1009 &   1263 &  0.44 \\
Other specified surgical operations and procedu... &   600 &    750 &  0.44 \\
Unspecified essential hypertension                 &  9370 &  11333 &  0.45 \\
Other iatrogenic hypotension                       &   953 &   1168 &  0.45 \\
Unspecified protein-calorie malnutrition           &   562 &    697 &  0.45 \\
Severe sepsis                                      &  1746 &   2166 &  0.45 \\
Intracerebral hemorrhage                           &   618 &    749 &  0.45 \\
Anemia in chronic kidney disease                   &   623 &    761 &  0.45 \\
Long-term (current) use of insulin                 &  1138 &   1400 &  0.45 \\
Long-term (current) use of anticoagulants          &  1709 &   2097 &  0.45 \\
Neonatal jaundice associated with preterm delivery &  1052 &   1212 &  0.46 \\
Acute posthemorrhagic anemia                       &  2072 &   2480 &  0.46 \\
Acute respiratory failure                          &  3473 &   4024 &  0.46 \\
Septic shock                                       &  1189 &   1397 &  0.46 \\
Chronic airway obstruction, not elsewhere class... &  2027 &   2404 &  0.46 \\
Diarrhea                                           &   484 &    565 &  0.46 \\
Pneumonia, organism unspecified                    &  2223 &   2616 &  0.46 \\
Need for prophylactic vaccination and inoculati... &  2680 &   3099 &  0.46 \\
Hematoma complicating a procedure                  &   566 &    658 &  0.46 \\
Other specified procedures as the cause of abno... &   693 &    809 &  0.46 \\
Other specified cardiac dysrhythmias               &  1137 &   1316 &  0.46 \\
Personal history of transient ischemic attack (... &   498 &    574 &  0.46 \\
Unspecified septicemia                             &  1702 &   2023 &  0.46 \\
Other convulsions                                  &   892 &   1042 &  0.46 \\
Acidosis                                           &  2127 &   2401 &  0.47 \\
Hypovolemia                                        &   641 &    733 &  0.47 \\
Congestive heart failure, unspecified              &  6106 &   7005 &  0.47 \\
Unspecified pleural effusion                       &  1281 &   1453 &  0.47 \\
Esophageal reflux                                  &  2990 &   3336 &  0.47 \\
Single liveborn, born in hospital, delivered wi... &  1668 &   1898 &  0.47 \\
Observation for suspected infectious condition     &  2570 &   2949 &  0.47 \\
Iron deficiency anemia secondary to blood loss ... &   482 &    530 &  0.48 \\
Hypoxemia                                          &   625 &    673 &  0.48 \\
Hyposmolality and/or hyponatremia                  &  1445 &   1594 &  0.48 \\
Mitral valve disorders                             &  1416 &   1510 &  0.48 \\
Encounter for palliative care                      &   485 &    535 &  0.48 \\
Personal history of venous thrombosis and embolism &   786 &    826 &  0.49 \\
Obesity, unspecified                               &   744 &    767 &  0.49 \\
Hypotension, unspecified                           &   996 &   1055 &  0.49 \\
Primary apnea of newborn                           &   506 &    537 &  0.49 \\
Intestinal infection due to Clostridium difficile  &   716 &    728 &  0.50 \\
Obstructive chronic bronchitis with (acute) exa... &   598 &    600 &  0.50 \\
Anemia of other chronic disease                    &   550 &    543 &  0.50 \\
Anemia, unspecified                                &  2729 &   2677 &  0.50 \\
Dehydration                                        &   704 &    681 &  0.51 \\
Other chronic pulmonary heart diseases             &  1101 &   1047 &  0.51 \\
Do not resuscitate status                          &   694 &    633 &  0.52 \\
Depressive disorder, not elsewhere classified      &  1888 &   1543 &  0.55 \\
Morbid obesity                                     &   648 &    522 &  0.55 \\
Iron deficiency anemia, unspecified                &   657 &    514 &  0.56 \\
Chronic diastolic heart failure                    &   708 &    532 &  0.57 \\
Hypopotassemia                                     &   816 &    609 &  0.57 \\
Anxiety state, unspecified                         &   944 &    636 &  0.60 \\
Asthma, unspecified type, unspecified              &  1317 &    878 &  0.60 \\
Dysthymic disorder                                 &   663 &    446 &  0.60 \\
Urinary tract infection, site not specified        &  4027 &   2528 &  0.61 \\
Other persistent mental disorders due to condit... &   698 &    428 &  0.62 \\
Acute on chronic diastolic heart failure           &   779 &    441 &  0.64 \\
Unspecified acquired hypothyroidism                &  3307 &   1610 &  0.67 \\
Osteoporosis, unspecified                          &  1637 &    310 &  0.84 \\
Personal history of malignant neoplasm of breast   &  1259 &     18 &  0.99 \\
\bottomrule
%%\end{tabular}
\caption{\todo{Add \% male} Condition name and gender balance for the ICD9 codes with at least 1000 observations in the \MIMIC dataset.}
\label{tab:top1000MIMIC}
\end{longtable*}
%%\end{table*}
